FoundLoc: Vision-based Onboard Aerial Localization in the Wild

Robust and accurate localization for Unmanned Aerial Vehicles (UAVs) is an essential capability to achieve autonomous, long-range flights. Current methods either rely heavily on GNSS, face limitations in visual-based localization due to appearance variances and stylistic dissimilarities between camera and reference imagery, or operate under the assumption of a known initial pose. In this paper, we developed a GNSS-denied localization approach for UAVs that harnesses both Visual-Inertial Odometry (VIO) and Visual Place Recognition (VPR) using a foundation model. This paper presents a novel vision-based pipeline that works exclusively with a nadir-facing camera, an Inertial Measurement Unit (IMU), and pre-existing satellite imagery for robust, accurate localization in varied environments and conditions. Our system demonstrated average localization accuracy within a $20$-meter range, with a minimum error below $1$ meter, under real-world conditions marked by drastic changes in environmental appearance and with no assumption of the vehicle's initial pose. The method is proven to be effective and robust, addressing the crucial need for reliable UAV localization in GNSS-denied environments, while also being computationally efficient enough to be deployed on resource-constrained platforms.

==> tables/table-DINO_profile.tex <==
\begin{table}[!t] % The [h] specifier suggests placing the table 'here' if possible
\centering % Centers the table on the page
\caption{Foundation model based VPR profile}
\scalebox{0.95}{
\begin{tabular}{cc}
\toprule
\textbf{Index} & \textbf{Profile} \\
\cmidrule{1-1} \cmidrule(lr{0.75em}){2-2}
\textbf{Platform} & NVIDIA Xavier NX \\

\textbf{Model Architecture} & DINO with ViT-S/8 \\

\textbf{Number of Parameters} & 21M \\

\textbf{Input Image Size} & $(500 \times 500) \rightarrow (224 \times 298)$ \\

\textbf{Feature Extraction Time (GPU)} & 0.517s / query \\

\textbf{Feature Extraction GPU Usage} & $>90\%$ \\

\textbf{VLAD Encoding Time (CPU)} & 0.107s / query \\

\textbf{VLAD Matching Time (CPU)} & 0.0018s /query \\
\bottomrule
\end{tabular}
}
\label{tab:DINO_profile}
\end{table}

==> tables/table-baseline_compare.tex <==
\begin{table}[h] % The [h] specifier suggests placing the table 'here' if possible
\centering % Centers the table on the page
\caption{Baseline Performance Comparison}
\scalebox{0.9}{
\begin{tabular}{lcccc}
\toprule
\textbf{Methods} & \textbf{Pattern} & \textbf{ATE [$m$]} & \textbf{Min Err. [$m$]} & \textbf{Max Err. [$m$]} \\
\cmidrule{1-1} \cmidrule(lr{0.75em}){2-2} \cmidrule(lr{0.75em}){3-5}
VIO + Initial Pose & \multirow{4}{*}{P. E.} &  44.66 & 3.49 & 57.57 \\

VIO + NetVLAD & & - & - & - \\

\coolname{}\textit{-NF} & & 115.25 & 0.53 & 358.6 \\

\rowcolor{Light}
\textbf{\coolname{}} & & 12.62 & 0.48 & 23.29 \\

\cdashmidrule{1-5}

VIO + Initial Pose & \multirow{4}{*}{P. R.} &  13.47 & 1.74 & 22.25 \\

VIO + NetVLAD & & - & - & - \\ 

% \rowcolor{Light}
\coolname{}\textit{-NF} & & 68.80 & 11.28 & 283.99  \\

\rowcolor{Light}
\textbf{\coolname{}} & & 12.57 & 0.31 & 34.51 \\
 
\bottomrule
\end{tabular}
}
\label{tab:Unit_test}
\end{table}

==> tables/table-different_alt.tex <==
% \begin{table}[!t] % The [h] specifier suggests placing the table 'here' if possible
% \centering % Centers the table on the page
% \caption{Test at different altitude}
% \scalebox{0.9}{
% \begin{tabular}{ccccc}
% \toprule 
%  \textbf{Pattern} & \textbf{Altitude [$m$]} & \textbf{ATE [$m$]} & \textbf{Min Err. [$m$]} & \textbf{Max Err. [$m$]} \\
% \cmidrule{1-1} \cmidrule(lr{0.75em}){2-2} \cmidrule(lr{0.75em}){3-5} 
% Eight & 50 & 9.926 & 1.54 & 15.56 \\

% Rectangle & 50& 12.146 & 1.12 & 31.67 \\
% \cdashlinelr{1-5}
% Eight & 75 & 17.198 & 0.74 & 45.58 \\

% Rectangle & 75 & 13.468 & 0.76 & 29.52 \\
% \cdashlinelr{1-5}
% Eight & 100 & 16.379 & 6.13 & 28.62 \\

% Rectangle & 100 & 35.38 & 2.44 & 52.23 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:Diff_alt}
% \end{table}

\begin{table}[!t] % The [h] specifier suggests placing the table 'here' if possible
\centering % Centers the table on the page
\caption{Test at different altitude}
\scalebox{0.9}{
\begin{tabular}{ccccc}
\toprule 
 \textbf{Pattern} & \textbf{Altitude [$m$]} & \textbf{ATE [$m$]} & \textbf{Min Err. [$m$]} & \textbf{Max Err. [$m$]} \\
\cmidrule{1-1} \cmidrule(lr{0.75em}){2-2} \cmidrule(lr{0.75em}){3-5} 
PE & 50 & 12.62 & 0.48 & 23.29 \\

PR & 50& 19.24 & 4.71 & 41.23 \\
\cdashlinelr{1-5}
PE & 75 & 22.39 & 0.74 & 38.99 \\

PR & 75 & 20.44 & 0.71 & 94.68 \\
\cdashlinelr{1-5}
PE & 100 & 25.77 & 7.89 & 74.00 \\

PR & 100 & 30.67 & 2.83 & 50.52 \\
\bottomrule
\end{tabular}
}
\label{tab:Diff_alt}
\end{table}

==> tables/table-different_condition.tex <==
% \begin{table}[!t] 
% \centering % Centers the table on the page
% \caption{Test at Different Environment Condition}
% \scalebox{0.9}{
% \begin{tabular}{cccc}
% \toprule
%  \textbf{Description} & \textbf{ATE [$m$]} & \textbf{Min Err. [$m$]} & \textbf{Max Err. [$m$]} \\
% \cmidrule(lr{0.75em}){1-1} \cmidrule(lr{0.75em}){2-4} 
%  June, Noon, Sunny & 12.146 & 1.12 & 31.67 \\

%  June, Afternoon, Cloudy & 14.242 & 1.24 & 30.34 \\

%  May, Noon, Sunny & 18.069 & 1.58 & 35.92 \\

%  May, Sunset, Sunny,  & 18.513 & 1.31 & 35.92 \\

%  July, Afternoon, Cloudy & 21.440 & 1.80 & 23.43 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:Diff_scene}
% \end{table}

% \begin{table}[!t] 
% \centering % Centers the table on the page
% \caption{Test at Different Environment Conditions.}
% \scalebox{0.9}{
% \begin{tabular}{cccc}
% \toprule
%  \textbf{Description} & \textbf{ATE [$m$]} & \textbf{Min Err. [$m$]} & \textbf{Max Err. [$m$]} \\
% \cmidrule(lr{0.75em}){1-1} \cmidrule(lr{0.75em}){2-4} 
% May, sunset, Sunny &  9.81 & 0.21 & 44.10 \\ %traj3, traj2 has gps issue
% May, Morning, Sunny & 22.97 & 3.20 & 107.65 \\ % traj5
% June, Noon, Sunny & 12.62 & 0.48 & 23.29 \\ %traj1
% June, Afternoon, Sunny & 19.54 & 5.10 & 57.65 \\ %traj4
% July, Afternoon, Cloudy & 13.85 & 1.06 & 26.45 \\ %traj6
% August, Afternoon, Rainy, Moving objects &  & & \\ 
% August, Night, Eight Pattern & 14.30 & 0.52 & 91.19 \\ % traj9
% August, Night, Rectangle Pattern &  32.80 & 0.58 & 203.9 \\ %traj10
% \cdashmidrule{1-4}
% Average & 1 & 2 & 3 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:Diff_scene}
% \end{table}


\begin{table*}[!t] 
\centering % Centers the table on the page
\caption{Flights Under Different Environmental Conditions.}
\scalebox{1}{
\begin{tabular}{cccccccc}
\toprule
& \multicolumn{4}{c}{\textbf{Conditions}} & \multicolumn{3}{c}{\textbf{Performance}} \\
\cmidrule(lr{0.75em}){2-5} \cmidrule(lr{0.75em}){6-8}

 \textbf{Sequence} & \textbf{Time} & \textbf{Pattern} & \textbf{Altitude} & \textbf{Weather} & \textbf{ATE [$m$]} & \textbf{Min Err. [$m$]} & \textbf{Max Err. [$m$]} \\
\cmidrule{1-1} \cmidrule(lr{0.75em}){2-2} \cmidrule(lr{0.75em}){3-3} \cmidrule(lr{0.75em}){4-4} \cmidrule(lr{0.75em}){5-5} \cmidrule(lr{0.75em}){6-6} \cmidrule(lr{0.75em}){7-7} \cmidrule(lr{0.75em}){8-8} 
1  & May, sunset       & P. E. & 50  & Sunny  & 9.810 & 0.21 & 44.10 \\ % exp4traj3, traj2 has gps issue
2  & May, Morning      & P. E. & 50  & Sunny  & 22.97 & 3.20 & 107.7 \\ % exp4traj5
3  & June, Noon        & P. E. & 50  & Sunny  & 12.62 & 0.48 & 23.29 \\ % exp4traj1
4  & June, Afternoon   & P. E. & 50  & Sunny  & 19.54 & 5.10 & 57.65 \\ % exp4traj4
5  & July, Afternoon   & P. E. & 50  & Cloudy & 13.85 & 1.06 & 26.45 \\ % exp4traj6
6  & July, Afternoon   & P. R. & 50  & Sunny  & 14.71 & 1.99 & 76.01 \\ % exp6traj2
7  & July, Afternoon   & P. E. & 75  & Sunny  & 22.39 & 0.74 & 38.99 \\ % exp2traj3
8  & July, Afternoon   & P. R. & 75  & Sunny  & 20.44 & 0.71 & 94.68 \\ % exp2traj4
9  & July, Afternoon   & P. E. & 100 & Sunny  & 25.77 & 7.89 & 74.00 \\ % exp2traj1
10 & July, Afternoon   & P. R. & 100 & Sunny  & 30.67 & 2.83 & 50.52 \\ % exp2traj2
11 & August, Afternoon & P. E. & 50  & Rainy  & 12.57 & 0.31 & 34.51 \\ % exp6traj1
12 & August, Night     & P. E. & 50  & Sunny  & 14.30 & 0.52 & 91.19 \\ % exp4traj9
13 & August, Night     & P. R. & 50  & Sunny  & 32.80 & 0.58 & 203.9 \\ % exp4traj10
\cdashmidrule{1-8}
\multicolumn{5}{c}{\textbf{Average}}  & 00 & 00 & 00 \\
\bottomrule
\end{tabular}
}
\label{tab:Diff_scene}
\end{table*}



==> tables/table-traj.tex <==
\begin{table}[!h] % The [h] specifier suggests placing the table 'here' if possible
\centering % Centers the table on the page
\caption{Baseline Flight Trajectory Setup}
\scalebox{1}{
\begin{tabular}{cccc}
\toprule 
& \multicolumn{3}{c}{\textbf{Properties}} \\
\cmidrule(lr{0.75em}){2-4}
\textbf{Pattern} & \textbf{Length [m]} & \textbf{Flight Speed [m/s]} & \textbf{AGL Alt. [m]} \\
\cmidrule{1-1} \cmidrule(lr{0.75em}){2-2} \cmidrule(lr{0.75em}){3-3} \cmidrule(lr{0.75em}){4-4}
Eight (PE) & 880 & 10 & 50 \\
Rectangle (PR) & 1000 & 10 & 50 \\
\bottomrule
\end{tabular}
}
\label{tab:trajs}
\end{table}

==> tables/table-unit_test.tex <==
% \begin{table}[h] % The [h] specifier suggests placing the table 'here' if possible
% \centering % Centers the table on the page
% \caption{Unit tests of pipeline performance}
% \scalebox{1}{
% \begin{tabular}{cccc}
% \toprule
%  \textbf{Pattern} & \textbf{ATE [$m$]} & \textbf{Min Err. [$m$]} & \textbf{Max Err. [$m$]} \\
% \cmidrule{1-1} \cmidrule(lr{0.75em}){2-4} 
% Eight & 9.926 & 1.54 & 15.56 \\

% Rectangle & 12.146 & 1.12 & 31.67 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:Unit_test}
% \end{table}

\begin{table}[h] % The [h] specifier suggests placing the table 'here' if possible
\centering % Centers the table on the page
\caption{Unit tests of pipeline performance}
\scalebox{1}{
\begin{tabular}{cccc}
\toprule
 \textbf{Pattern} & \textbf{ATE [$m$]} & \textbf{Min Err. [$m$]} & \textbf{Max Err. [$m$]} \\
\cmidrule{1-1} \cmidrule(lr{0.75em}){2-4} 
PE &  12.62 & 0.48 & 23.29 \\

PR & 19.24 & 4.71 & 41.23 \\
\bottomrule
\end{tabular}
}
\label{tab:Unit_test}
\end{table}



==> text/06-implementation.tex <==
\section{Implementation details}
